Fast and Robust Fixed-Rank Matrix Recovery

We address the problem of efficient sparse fixed-rank (S-FR) matrix decomposition, i.e., splitting a corrupted matrix $M$ into an uncorrupted matrix $L$ of rank $r$ and a sparse matrix of outliers $S$. Fixed-rank constraints are usually imposed by the physical restrictions of the system under study. Here we propose a method to perform accurate and very efficient S-FR decomposition that is more suitable for large-scale problems than existing approaches. Our method is a grateful combination of geometrical and algebraical techniques, which avoids the bottleneck caused by the Truncated SVD (TSVD). Instead, a polar factorization is used to exploit the manifold structure of fixed-rank problems as the product of two Stiefel and an SPD manifold, leading to a better convergence and stability. Then, closed-form projectors help to speed up each iteration of the method. We introduce a novel and fast projector for the $\text{SPD}$ manifold and a proof of its validity. Further acceleration is achieved using a Nystrom scheme. Extensive experiments with synthetic and real data in the context of robust photometric stereo and spectral clustering show that our proposals outperform the state of the art.

==> sections/Approach_back.tex <==
\section{Sparse Fixed-Rank Decomposition}
\label{sec:approach}

We propose the resolution of the non-convex program in (\ref{eq:decomp}) as a direct way to perform the sparse and fixed-rank decomposition\footnote{Notice that (\ref{eq:decomp}) is analogous to the program (\ref{eq:fr}) defined in Sec.\ref{sec:intro}}. The optimization of (\ref{eq:decomp}) is carried out over an Augmented Lagrange function, leading to the expression shown in (\ref{eq:lagrange}). $Y$ stands for the Lagrange multiplier and $\mathcal{F}^{(r)}_{m,n}$ represents the fixed-rank manifold of rank $r$.

\vspace{-6mm}
\begin{equation}
\label{eq:decomp}
\text{min}_{L, S} \norm{S}_{\ell_1}, s.t.\  M = L + S,\  L \in \mathcal{F}^{(r)}_{m,n},
\end{equation}

\vspace{-7mm}
\begin{equation}
\scalemath{0.81}{
\mathcal{L}(L, S, Y, \mu) = \frac{1}{\mu}\norm{M-L-S}_F^2 + \lambda \norm{S}_{\ell_1} + \langle Y, M-L-S \rangle. \nonumber
}\end{equation}
\vspace{-7mm}
\begin{equation}
\label{eq:lagrange}
s.t. L \in \mathcal{F}^{(r)}_{m,n}
\end{equation}

To efficiently solve (\ref{eq:lagrange}) we utilize an ADM scheme~\cite{ALM} endowed with a continuation step, as presented in Algorithm~\ref{ADM}. The update of the fixed-rank matrix $L$ is obtained via the FixedRankOpt algorithm that implements the proposed polar factorization. For the sparse matrix $S$, the standard soft-thresholding is used. Notice that $\mu_k$ is updated following a geometric series in order to achieve a Q-linear converge rate $O(1/\mu_k)$~\cite{ALM}. Despite presenting the same asymptotic convergence order than AS, our method converges faster. Given sequence $\{\rho \mu_k\}_{k=1}^{k_{\text{max}}}$ for the continuation, then the convergence of FR-ADM follows $\sim C_{\text{FR}} g(\rho \mu_k)$  and AS follows $\sim C_{\text{AS}} g(\rho \mu_k)$, for a common function  $g(\rho\mu_k) = \frac{1}{\rho \mu_k}$. Comparing the constants of both methods  we have that $\frac{ C_{\text{FR}} }{  C_{\text{AS}} } << 1$. We provide empirical validation for this claim in Sec.~\ref{sec:results}, by counting the number of iterations up to convergence.

\setlength{\textfloatsep}{10pt}
\begin{algorithm}
 \algsetup{linenosize=\small}
  \small
\begin{algorithmic}
        \REQUIRE Data matrix $M\in \mathbb{R}^{m\times n}$
    \STATE $k \leftarrow 1, S_k \leftarrow 0_{m \times n}, L_k \leftarrow 0_{m \times n}, Y_k \leftarrow 0_{m \times n}$
    \STATE $\mu_k \leftarrow 1, \rho > 1, \bar{\mu} \leftarrow 10^9, U_0 \leftarrow I_{m \times r}, B_0 \leftarrow I_{r}, V_0 \leftarrow I_{r \times n}$
    \vspace{-2mm}
    \WHILE{not converged}
	\STATE $L_{k+1} \leftarrow \textrm{arg min}_{L\in \mathcal{F}_r} \mathcal{L}(L, S_k, Y_k, \mu_k)$
	\STATE \ \ \  \ \  \  \  \  \ \  \ $= \textit{FixedRankOpt}(M - S_k + \frac{1}{\mu_k} Y_k, U_0, B_0, V_0)$
	\STATE $S_{k+1} \leftarrow \textrm{arg min}_{S\in \mathbb{R}^{m \times n}} \mathcal{L}(L_{k+1}, S, Y_k, \mu_k)$
	\STATE \ \ \  \ \  \  \  \  \ \  \ $= \text{Soft}(M - L_{k+1} +  \frac{1}{\mu_k} Y_k)$
	\STATE $Y_{k+1} \leftarrow Y_k + \mu_k (M - L_{k+1} - S_{k+1})$
	\STATE $\mu_{k+1} \leftarrow \text{min}(\bar{\mu}, \rho \mu_k)$
	\STATE $k \leftarrow k + 1$
	\ENDWHILE
	\RETURN{$L_k$, $S_k$.}
\end{algorithmic}
\caption{FixedRank-ADM}
\label{ADM}
\end{algorithm}

\subsection{Polar Factorization in the Fixed-Rank Manifold}
\label{sec:polar}

When dealing with rank constraints, we need an efficient way of computing the projection of an arbitrary matrix  $M \in \mathbb{R}^{m \times n}$ with arbitrary rank onto the fixed-rank manifold $\mathcal{F}^{(r)}_{m,n}$. For this task, a simple solution is provided by the EckartÃ¢â‚¬â€œYoung theorem~\cite{SVD}, which shows that the optimization problem (\ref{eq:Eck}):
%
\begin{equation}
\textrm{min}_{\textrm{rank}(L)= r}\norm{M-L}_F^2,
\label{eq:Eck}
\end{equation}
%
\noindent is solved by the truncated SVD (TSVD) of $M$, $L=U\Sigma V^T$, where $U\in \textrm{St}_{m,r},U^TU=I_r$, 
$V\in \textrm{St}_{n,r},V^TV=I_r$ and $\Sigma$ is a diagonal matrix with positive entries given by the first $r$ singular values of $M$. 

Despite the great success of the TSVD as a tool to produce low-rank approximations, some problems require the computation of many TSVDs (typically one per iteration) of very large matrices, and therefore an efficient alternative to the usual TSVD algorithm is required. In this section we propose the method \textit{FixedRankOpt} (Algorithm~\ref{Alg-FROpt}), which computes the projection of a matrix onto the fixed-rank manifold, leading to the optimal solution of the TSVD.  Our method shows a convergence rate of $O(\log(1/\epsilon))$, converging in a small fraction of the time taken by a TSVD. Additionally, we also propose the method \textit{FixedRankStep} (Algorithm~\ref{Alg-FRStep}) as a part of the more general  \textit{FixedRankOpt}. \textit{FixedRankOpt} can be seen as a series of iterations of the \textit{FixedRankStep} algorithm, which provides a proximal solution to the TSVD, with solutions living on $\mathcal{F}^{(r)}_{m,n}$, but much cheaper than the standard TSVD. The \textit{FixedRankStep} algorithm is suitable for large-scale problems, where many TSVD of large matrices are required. Notice that exact projections do not need to be computed in each iteration. In a sense, \textit{FixedRankOpt} performs an exact line-search in the normal direction towards the fixed-rank manifold, while \textit{FixedRankStep} performs an inexact line-search in the same direction. In many cases an inexact line-search is fast and enough to ensure convergence, as we will show later.

Following~\cite{Meyer}, we shall consider a polar factorization on $\mathcal{F}^{(r)}_{m,n}$ given by the TSVD,  which will turn very convenient. Given a matrix $L \in \mathbb{R}^{m \times n}$ of rank $r$, its TSVD factorization is $L=U\Sigma V^T$, where $U\in \textrm{St}_{m,r},U^TU=I_r$, $V\in \textrm{St}_{n,r},V^TV=I_r$ and $\Sigma$ is a diagonal $r\times r$ matrix with positive entries. A transformation $(U,\Sigma, V)\rightarrow (U O,O^T\Sigma O, V O)$, where $O\in O_r$ is an orthogonal matrix, does not change $L$, and allows to write it as $L=UB V^T$, where now $B\in \textrm{SPD}_r$. Therefore, the fixed-rank manifold can be seen as the quotient manifold $(\textrm{St}_{m,r}\times \textrm{SPD}_r\times \textrm{St}_{n,r})/O_r$. From this, we reformulate the problem of minimizing $M$ in the fixed-rank manifold as the solution of (\ref{eq:MinimizationFixedRank}).
\vspace{-3mm}
\begin{equation}
\textrm{min}_{U\in \textrm{St}_{m,r},B\in \textrm{SPD}_r,V\in \textrm{St}_{n,r}}\norm{M-UB V^T}_F^2.
\label{eq:MinimizationFixedRank}
\end{equation}
\vspace{-5mm}

The program (\ref{eq:MinimizationFixedRank}), although highly non-convex, converges geometrically to the global minimum when optimized via the proposed \textit{FixedRankOpt} method (Algorithm~\ref{Alg-FROpt}). The input matrices $U_0$, $B_0$ and $V_0$ are initialized as previously mentioned in Algorithm~\ref{ADM}.

\vspace{-1mm}
%\setlength{\textfloatsep}{0pt}
\begin{algorithm}
 \algsetup{linenosize=\small}
  \small
\begin{algorithmic}
        \REQUIRE Data matrix $M\in \mathbb{R}^{m\times n}$, inital matrices $U_0\in \textrm{St}_{m,r}$, $B_0\in \textrm{SPD}_r$, $V_0\in \textrm{St}_{n,r}$
	\STATE $i\leftarrow 0$
	\WHILE{not converged}
	\STATE $(U_{i+1},B_{i+1},V_{i+1})\leftarrow FixedRankStep(M,U_i,B_i,V_i)$
	\STATE $i\leftarrow i+1$
	\ENDWHILE
	\RETURN{$U^*\in \textrm{St}_{m,r}$, $B^*\in \textrm{SPD}_r$, $V^*\in \textrm{St}_{n,r}$ such that $L=U^*B^*{V^*}^T$ is the 
	TSVD of $M$ }
\end{algorithmic}
\caption{FixedRankOpt Algorithm}
\label{Alg-FROpt}
\end{algorithm}
\vspace{-2mm}

Here, the \textit{FixedRankStep} algorithm performs an alternating directions minimzation (ADM)
on each of the submanifolds $\textrm{St}_{m,r}$, $\textrm{St}_{n,r}$ and $\textrm{SPD}_r$, as shown in Algorithm~\ref{Alg-FRStep}
\vspace{-1mm}

\setlength{\textfloatsep}{3pt}
\begin{algorithm}
 \algsetup{linenosize=\small}
  \small
\begin{algorithmic}
        \REQUIRE Data matrix $M\in \mathbb{R}^{m\times n}$, previous values $U_0\in \textrm{St}_{m,r}$, $B_0\in \textrm{SPD}_r$, $V_0\in \textrm{St}_{n,r}$
	\STATE $U \leftarrow \textrm{arg min}_{U\in \textrm{St}_{m,r}}\norm{M-UB_0 V_0^T}_F^2$
	\STATE $V \leftarrow \textrm{arg min}_{V\in \textrm{St}_{n,r}}\norm{M-UB_0 V^T}_F^2$
	\STATE $B \leftarrow \textrm{arg min}_{B\in \textrm{SPD}_r}\norm{M-UB V^T}_F^2$	
	\RETURN{$U\in \textrm{St}_{m,r}$, $B\in \textrm{SPD}_r$, $V\in \textrm{St}_{n,r}$. }
\end{algorithmic}
\caption{FixedRankStep Algorithm}
\label{Alg-FRStep}
\end{algorithm}
\vspace{-2mm}

In our formulation, we are dealing with minimization subproblems on the Stiefel manifold that are not those of the standard  Stiefel Procrustes Problem~\cite{Stiefel-Procrustes}. In our case the Stiefel matrix is left-multiplying instead of right-multiplying, as usually assumed. Fortunately, this change turns out to allow us to produce a fast closed-form solution by using the well-known Orthogonal Procrustes Problem (OPP)~\cite{Orth-Procrustes}, as shown in (\ref{eq:OrthogonalProcrustes}):

\vspace{-5mm}
\begin{equation}
\textrm{min}_{U\in \textrm{St}_{m,r}}\norm{M-UBV^T}_F^2 \Rightarrow\quad U=P_{\textrm{O}}[MVB] ,
\label{eq:OrthogonalProcrustes}
\end{equation}
%
where $P_{\textrm{O}}[A]$ is the projector onto the Stiefel Manifold (i.e. the column space of $A$), and can be efficiently computed through an SVD as $A= Q\Sigma S^T \,,Q\in\textrm{St}_{m,r}\,,S\in O_r \Rightarrow  U=QS^T$.

A similar result holds for the minimization of $V$ by simply transposing (\ref{eq:OrthogonalProcrustes}). Note that there exists an explicit solution for the double Orthogonal Procrustes Problem ~\cite{MatrixProcrustesProblems}, but it requires the computation of the TSVD of $M$, something that would be computationally expensive, and it is not applicable in the  Stiefel case.

The minimization subproblem on the SPD manifold is more challenging. The reason is that, although convex, the SPD manifold is an open manifold and therefore the existence of a global minimum in not guaranteed. Its closure is the SPSD manifold, and there the existence of a solution is neither guaranteed. However, we shall see that in our case there exists a minimun in $\text{SPD}_r$. Let us analyse this by first introducing a novel projector onto the SPD manifold. To this end we consider the SPD Procrustes Problem~\cite{SPDProcrustes} (\ref{SPDProcrustes}):

\vspace{-5mm}
\begin{equation}
\scalemath{0.98}{
\textrm{min}_{B\in \textrm{SPD}_r}\norm{M-UBV^T}_F^2 \Rightarrow  B=P_{\textrm{SPD}}[U^TMV],}
\label{SPDProcrustes}
\end{equation}
\vspace{-4mm}

\noindent where the projector $P_{\textrm{SPD}}[A]$ is simply given by $P_{\textrm{SPD}}[A]=\textrm{Sym}(A)$. In general, the solution of the SPD Procrustes Problem requires to solve a Lyapunov equation~\cite{SPDProcrustes}, but in our case is simpler since $U$ and $V$ are orthogonal. Although in general, there is not guarantee that $B=\textrm{Sym}(U^TMV)$ is positive definite, we can assure it for our formulation. Given that $\text{rank}(M) > r = \text{rank}(L)$, and considering $U$ and $V$ as the solutions of an OPP, then a unique solution in the SPD manifolds must exist. This solution is given in the following discussion, but we need some previous results.

\begin{lem}
 (see \cite{Stiefel-Procrustes}) Let $U$ (or $V$) be the solution of the OPP (\ref{eq:OrthogonalProcrustes}), then $U^TMVB$ (or $BU^TMV$) is in $\textrm{SPD}_r$.
\label{lemmaOPP}
\end{lem}

\vspace{-3mm}
\noindent \textit{Proof}: As shown before, if $MVB=Q\Sigma S^T$, then $U=QS^T$ and $U^TMVB=SQ^TQ\Sigma S^T=S\Sigma S^T$, which is SPD since $\textrm{rank}(M)\geq r$ and $B$ is supposed to be in $\textrm{SPD}_r$. A similar argument shows that $BU^TMV \in \textrm{SPD}_r$ after minimizing $V$.

%\vspace{-2mm}
From Lemma~\ref{lemmaOPP}, we have that $U_{i+1}^TMV_iB_i$ and $B_iU_{i+1}^TMV_{i+1}$ are in $SPD_r$, but in order to proof $B_{i+1}=\textrm{Sym}(U_{i+1}^TMV_{i+1})\in \textrm{SPD}_r$ we need to pass to the limit. When passing to the limit the sequences defined by $\{U_i\}$, $\{B_i\}$ and $\{V_i\}$, it can be seen that both conditions are simultaneously met, as presented in Lemma~\ref{lemmaSPDLimit}:

\vspace{-2mm}
\begin{lem}
Suppose that the \textit{FixedRankOpt} Algorithm converges to a fixed point $(U^*,B^*,V^*)$, then
$U^*\in \textrm{St}_{m,r}$, $B^*\in \textrm{SPD}_r$, and $V^*\in \textrm{St}_{n,r}$.
\label{lemmaSPDLimit}
\end{lem}

\vspace{-1mm}
\noindent \textit{Proof}: Since $\scalemath{0.92}{(U^*,B^*,V^*)=\textit{FixedRankStep}(M,U^*,B^*,V^*)}$, $U^*$ and $V^*$ are solutions to their respective OPPs and have to be in their respective Stiefel manifolds. Then, by applying Lemma~\ref{lemmaOPP}, both $U^*{}^TMV^*B^*$ and $B^*U^*{}^TMV^*$ are in SPD$_r$. Since $B^*=\textrm{Sym}(U^*{}^TMV^*)$, it can be derived that:\newline

\setlength{\abovedisplayskip}{-4mm}
\begin{eqnarray}
 2B^*{}^2 &=& B^*\textrm{Sym}(U^*{}^TMV^*)+\textrm{Sym}(U^*{}^TMV^*)B^* \nonumber\\
&=& U^*{}^TMV^*B^*+B^*U^*{}^TMV^*\,,
\end{eqnarray}

\noindent which is on SPD$_r$ since it is a convex manifold. Then, by taking the square root of $B^*{}^2$ we have that 
$B^*\in \textrm{SPD}_r$. Also, since $\textrm{SPD}_r$ is open in the subset of symmetric matrices, there exists $\epsilon>0$ such that the open ball of radius $\epsilon$ is contained in $\textrm{SPD}_r$. Thus, if \textit{FixedRankOpt} converges, then there exists $n_0\in \mathbb{N}$ such that $B_i\in \textrm{SPD}_r\,\forall i\geq n_0$. In fact in our numerical experiments we always have that $B_i\in \textrm{SPD}_r\,\forall i\geq 1$. The actual value of $B_0$ does not really matter, and we always take $B_0=I_r$. From this, Theorem~\ref{TheoremGlobalMinimum} assures the convergence of the \textit{FixedRankOpt} algorithm for arbitrary initial matrices $U_0\in \textrm{St}_{m,r}$, $B_0\in \textrm{SPD}_r$, $V_0\in \textrm{St}_{n,r}$:

\begin{thm}
The \textit{FixedRankOpt} Algorithm converges to the unique global minimun of (\ref{eq:MinimizationFixedRank}) given by $(U^*,B^*,V^*)$ such that $L=U^*B^*V^*{}^T$ is the rank-r projection of $M$.
\label{TheoremGlobalMinimum}
\end{thm}

\vspace{-3mm}
Due to space limitations the  proof of this theorem is supplied as additional material. We shall only mention that our proof of convergence is based on the three points property and the fact that the Stiefel manifold is compact, and therefore the sequences $\{U_i\}$ and $\{V_i\}$ admit sub-sequences $\{U_{s_i}\}$ and  $\{V_{s_i}\}$ converging to some $\hat{U}$ and $\hat{V}$. Then, the subsequence $B_{s_i}=\textrm{Sym}(U_{s_i}^TMV_{s_i})$ also converges to some $\hat{B}$. From this we prove that $(\hat{U}, \hat{B},\hat{V})$ is the unique fixed-point of the iterative algorithm, minimizing the problem (\ref{eq:MinimizationFixedRank}), and thus providing the solution $(U^*,B^*,V^*)=(\hat{U}, \hat{B},\hat{V})$.

The \textit{FixedRankStep} algorithm produces by itself a good approximation of $M$ to a rank-r matrix $L$, provided that the initial estimates $U_0,B_0,V_0$ are well chosen. Since this is a modification of the orthogonal iteration from the computations of eigenvalues~\cite{MatrixComputations}, in each iteration the error $\norm{L^*-UBV^T}_F$ is decreased by a factor $(\frac{\sigma_{r+1}}{\sigma_r})$, where $\sigma_i$ are the singular values of $M$~\cite{MatrixComputations}. Given that $M$ is of the form $M=L+S$, with $L \in \mathcal{F}^{(r)}_{m,n}$ and $S$ is a perturbation matrix, then $\sigma_{r+1}$ will be much smaller than $\sigma_{r}$ and the error will be largely decreased in each iteration.

In the \textit{FixedRankOpt} algorithm, the initial matrices $U_0$ and $V_0$ must satisfy that their respective column spaces intersect with the ones of the optimal solution $L=U^*B^*{V^*}^T$ but, due to the form of the solution of the OPP, it is possible to choose, without loss of generality, $U_0 = I_{m\times r}$, $V_0 = I_{n \times r}$ and $B_0=I_r$. From this selection, the error of \textit{FixedRankOpt} after $k$ iterations is bounded by by $(\frac{\sigma_{r+1}}{\sigma_r})^{k}$, which leads to a Q-linear rate of convergence with order $O(log(1/\epsilon))$ to achieve a given error  $\epsilon$.

It is worth mentioning that the \textit{FixedRankOpt} algorithm, for the case $r=1$ can be seen as a two-step
version of the Power Method. In this context, the \textit{FixedRankStep} algorithm first obtains an approximation of the left and right dominant eigenvectors, $u_{i+1}=\frac{Mv_i}{\norm{Mv_i}_2}$, $v_{i+1}=\frac{M^Tu_{i+1}}{\norm{M^Tu_{i+1}}_2}$, and finally an approximation of the dominant singular value $b_{i+1}=u_{i+1}^TMv_{i+1}$ of $M$, which is strictly positive due to Lemma \ref{lemmaOPP}.

==> sections/Problem.tex <==
\section{Problem formulation}
\label{sec:problem}

